LearnedFTL: A Learning-Based Page-Level FTL for Reducing Double Reads in Flash-Based SSDs

We present LearnedFTL, a new on-demand page-level flash translation layer (FTL) design, which employs learned indexes to improve the address translation efficiency of flash-based SSDs. The first of its kind, it reduces the number of double reads induced by address translation in random read accesses. LearnedFTL proposes three key techniques: an in-place-update linear model to build learned indexes efficiently, a virtual PPN representation to obtain contiguous PPNs for sorted LPNs, and a group-based allocation and model training via GC/rewrite strategy to reduce the training overhead. By tightly integrating the aforementioned key techniques, LearnedFTL considerably speeds up address translation while reducing the number of flash read accesses caused by the address translation. Our extensive experiments on a FEMU-based prototype show that LearnedFTL can reduce up to 55.5\% address translation-induced double reads. As a result, LearnedFTL reduces the P99 tail latency by 2.9$\times$ $\sim$ 12.2$\times$ with an average of 5.5$\times$ and 8.2$\times$ compared to the state-of-the-art TPFTL and LeaFTL schemes, respectively.

==> sections/5-Related_Work.tex <==

\section{Related Work}
\label{related}

\subsection{Mapping Schemes in FTL Design}

Existing address mapping schemes in flash-based SSDs can be classified into three categories: (1) page-level mapping, (2) block-level mapping, and (3) hybrid mapping. A survey paper~\cite{FTLSurvey} provides a broad overview of some typical address translation technologies for flash memories~\cite{gupta2009dftl,qin2011two,jiang2011s,wang2012zftl}. Among them, page-level mapping shows the best performance due to fine-grained mapping, but it requires a large mapping table~\cite{zhou2015efficient,chen2019hcftl,zhou2018correlation,mativenga2019rftl,ni2017hash,han2019wal,chen2019beyond,GFTL}. The existing mapping schemes share a common design principle: exploiting the workload locality to selectively cache a small part of mapping entries in DRAM while storing the whole mapping table on flash. As a result, they work well under workloads with strong access locality. However, if the working set is too large or accesses are random, the cache hit ratio will be very low and the performance will degrade significantly due to frequent swapping operations and double reads~\cite{zhou2015efficient}.


%Existing address mapping schemes in flash-based SSDs can be classified into three categories: (1) page-level mapping, (2) block-level mapping, and (3) hybrid mapping. 

%Among all mapping granularities, page-level mapping shows the best performance due to fine-grained mapping, but it requires a large mapping table. Some demand-based page-level FTL schemes were proposed to speed up the address translation with a limited size of DRAM~\cite{gupta2009dftl,qin2011two,thontirawong2014scftl,jiang2011s,zhou2015efficient,chen2019hcftl,wang2012zftl,zhou2018correlation,mativenga2019rftl,GFTL,zhang2019reinforcement,ni2017hash,chen2019beyond}. DFTL~\cite{gupta2009dftl}, the first demand-based page-level FTL, shows a great improvement over hybrid FTL designs. Its subsequent variants, such as TPFTL and HCFTL~\cite{chen2019hcftl}, focus on the optimization of cache replacement and management to further improve the hit ratio of mapping cache and the performance of flash-based SSDs. 

Recent studies also utilize machine learning (ML) techniques to improve the performance of flash-based SSDs~\cite{yang2019reducing,akgun2021machine,kang2017reinforcement,zhang2019reinforcement,LearnedSSD}. For example, Q-FTL~\cite{zhang2019reinforcement} uses a reinforcement learning-driven cache replacement algorithm to adapt and respond to ever-changing I/O streams, but only for specific workloads, i.e., remote sensing datasets. LearnedSSD~\cite{LearnedSSD} accelerates the development of new SSD devices by automating the hardware parameter configurations by utilizing both supervised and unsupervised ML techniques. Yang et al.~\cite{yang2019reducing} reduced GC overhead in SSD by introducing ML techniques to predict the future temperature of data. However, none of them have considered ML-based methods on the address mapping optimizations within flash-based SSDs.


\subsection{Learned Index}
% \vspace{-3pt}

Learned index builds an explicit model of the underlying data to provide effective indexing. It was first introduced in~\cite{kraska2018case} and many learned indexes have been proposed based on the idea, such as PGM index~\cite{ferragina2020pgm}, FITing tree~\cite{FITing}, ALEX~\cite{ALEX}, Flood~\cite{Flood}, Tsunami~\cite{Tsunami}, and FINEdex~\cite{li2021finedex}. They all investigate how to support update capability, provide better worst-case guarantees, and/or efficient index construction for different workloads.

Recently, BOURBON~\cite{Bourbon} shows how to integrate learned index structure for an LSM-based KV store. BOURBON employs greedy piecewise linear regression to learn key distributions and applies a cost-benefit strategy to decide when learning will be worthwhile, thus enabling fast lookup with minimal computation. APEX~\cite{APEX} is a PM-optimized learned index based on ALEX~\cite{ALEX}. APEX retains the benefits of learned indexes while guaranteeing crash consistency on PM and supporting instant recovery and scalable concurrency. Abu-Libdeh et al.~\cite{BigTable} demonstrate how a learned index can be integrated into a distributed and disk-based database system, Google’s Bigtable. Their results also validate that integrating the learned index can significantly improve the end-to-end read latency and throughput for Bigtable.

Inspired by these advancements in the learned index techniques, LearnedFTL is the first study on leveraging the learned index to improve the page-level FTL designs of flash-based SSDs to accelerate the address translation for workloads with random accesses. Different from the aforementioned learned index techniques, LearedFTL exploits the GC characteristics of flash devices to relocate physical flash pages and a virtual PPN representation to satisfy the training requirements of the learned index. Moreover, it eliminates the error interval associated with the traditional learned index with the bitmap prediction filter to reduce read amplification in flash storage.

